Assessing the Creativity of LLMs in Proposing Novel Solutions to Mathematical Problems

The mathematical capabilities of AI systems are complex and multifaceted. Most existing research has predominantly focused on the correctness of AI-generated solutions to mathematical problems. In this work, we argue that beyond producing correct answers, AI systems should also be capable of, or assist humans in, developing novel solutions to mathematical challenges. This study explores the creative potential of Large Language Models (LLMs) in mathematical reasoning, an aspect that has received limited attention in prior research. We introduce a novel framework and benchmark, CreativeMath, which encompasses problems ranging from middle school curricula to Olympic-level competitions, designed to assess LLMs' ability to propose innovative solutions after some known solutions have been provided. Our experiments demonstrate that, while LLMs perform well on standard mathematical tasks, their capacity for creative problem-solving varies considerably. Notably, the Gemini-1.5-Pro model outperformed other LLMs in generating novel solutions. This research opens a new frontier in evaluating AI creativity, shedding light on both the strengths and limitations of LLMs in fostering mathematical innovation, and setting the stage for future developments in AI-assisted mathematical discovery.

==> 1_introduction.tex <==
\section{Introduction}

In recent years, artificial intelligence has made significant strides, particularly in the development of Large Language Models (LLMs) capable of tackling complex problem-solving tasks. Models like GPT-4 and Gemini-1.5-Pro have demonstrated impressive proficiency on rigorous mathematical benchmarks such as GSM8K \citep{cobbe2021training} and MATH \citep{hendrycks2021measuring}, underscoring the evolving role of LLMs from simple text generators to sophisticated tools capable of engaging with high-level mathematical challenges. However, while these models have excelled in achieving high accuracy on established mathematical datasets, their potential for creative problem-solving remains underexplored.

Mathematical creativity goes beyond solving problems correctly; it involves generating novel solutions, applying unconventional techniques, and offering deep insights—areas traditionally associated with human ingenuity. Yet, most studies have focused primarily on correctness and efficiency, paying little attention to the innovative approaches LLMs might employ. Furthermore, creativity in mathematical problem-solving is rarely integrated into existing benchmarks, limiting our understanding of LLMs' full potential. The current research landscape lacks a comprehensive framework that evaluates both the accuracy and the creative capacity of LLMs. This gap highlights the need for new methodologies and benchmarks specifically designed to assess and cultivate the creative problem-solving abilities of LLMs in mathematics, which is the focus of this paper.

%In recent years, the field of artificial intelligence has witnessed significant advancements in the capabilities of Large Language Models (LLMs) to address complex problem-solving tasks. Notably, models such as GPT-4 and Gemini-1.5-Pro have demonstrated impressive proficiency on rigorous mathematical benchmarks like the GSM8K \citep{cobbe2021training} and MATH \citep{hendrycks2021measuring} datasets. These achievements highlight the evolving role of LLMs from mere textual generators to sophisticated analytical tools capable of engaging with and solving high-level mathematical challenges. However, the application of LLMs extends beyond their ability to solve problems correctly; it also encompasses the exploration of their potential for creative problem-solving. Mathematical creativity, particularly in problem-solving contexts, involves the generation of novel solutions, the application of unconventional problem-solving techniques, and the provision of deep insights into the problems at hand. While LLMs have proven their competence in standard mathematical tasks, their capacity for innovation and creativity in mathematics—a domain traditionally associated with human ingenuity—remains underexplored.


%Despite their demonstrated success in achieving high accuracy on established mathematical datasets, the ability of LLMs to transcend traditional solution pathways and exhibit genuine creativity remains insufficiently examined. Most existing studies have primarily focused on the correctness and efficiency of solutions, with less attention given to the processes and novel approaches that LLMs might employ. Moreover, the assessment of creativity in mathematical problem-solving has not been systematically integrated into the benchmarks used to evaluate these models. This oversight limits our understanding of the full spectrum of capabilities that LLMs can offer. The current research landscape lacks a comprehensive framework that not only measures the accuracy of solutions provided by LLMs but also critically evaluates their ability to innovate and generate solutions that are both novel and valuable. 
%This gap in research highlights the need for new methodologies and benchmarks specifically designed to assess and cultivate the creative problem-solving potential of LLMs in the realm of mathematics, which is the focus of this paper. 

We created the dataset \textbf{CreativeMath}, a comprehensive math benchmark that includes problems from middle school to Olympic-level competitions, each accompanied by multiple high-quality solutions ranging from straightforward to highly innovative approaches. Additionally, we designed a multi-stage framework to rigorously evaluate the creativity of LLMs in generating novel math solutions. This evaluation spans closed-source, open-source, and math-specialized LLMs, assessing both the correctness and novelty of their solutions based on different reference prior solutions. 

%Our evaluation yields interesting insights: (1) 
%Gemini-1.5-Pro stood out in generating unique solutions, with nearly all correct solutions being distinct from the provided references. In contrast, smaller and math-specialized models struggled to produce novel solutions. (2) Providing more reference solutions generally improved the accuracy of LLMs. For instance, Gemini-1.5-Pro achieved perfect accuracy when given four prior solutions. However, as more solutions were provided, the models found it harder to generate new, unique solutions, reflecting a trade-off between using existing knowledge and fostering creativity. (3) As the difficulty of math problems increased, LLM accuracy decreased. However, when these models did solve harder problems, they were more likely to generate innovative solutions, suggesting that challenging problems push models toward more creative approaches. (4) Analyzing the similarity between solutions generated by different LLMs revealed that some models, like Llama-3-70B and Yi-1.5-34B, explored very different approaches, while others, like Mixtral-8x22B, tended to produce more similar solutions to other models. Using a diverse set of LLMs can therefore enhance the range and originality of generated solutions.

Our evaluation revealed several interesting key insights: (1) Gemini-1.5-Pro excelled in generating unique solutions, with most correct answers being distinct from the provided references, while smaller and math-specialized models struggled with novelty. (2) Providing more reference solutions generally improved accuracy, with Gemini-1.5-Pro achieving perfect accuracy with four prior solutions. However, increased references made it harder for models to generate unique solutions, indicating a trade-off between leveraging existing knowledge and fostering creativity. (3) As math problem difficulty increased, LLM accuracy declined, but successful solutions were more likely to be innovative, suggesting that tougher problems encourage creativity. (4) Analysis of solution similarity among different LLMs showed that models like Llama-3-70B and Yi-1.5-34B explored diverse approaches, while others like Mixtral-8x22B produced more similar solutions, highlighting the value of using a diverse set of LLMs to enhance originality.

This study lays the groundwork for future advancements in LLM math creativity. The major contributions include: (1) Introducing a new task—evaluating LLMs' mathematical creativity, (2) Creating the CreativeMath dataset, (3) Developing a framework for assessing mathematical creativity in LLMs, and (4) Evaluating state-of-the-art LLMs, revealing key insights into their strengths and limitations.

% Through extensive experiments and analyses, we evaluate ten leading LLMs, including both open-source and closed-source models, to determine their ability to generate novel solutions in the context of mathematical problem-solving. Our findings reveal significant variations in the creativity of these models, with some demonstrating a remarkable ability to produce original solutions that surpass human ingenuity.

==> images/images.tex <==
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.5\textwidth]{AnonymousSubmission/LaTeX/images/Twosets_Counts_Bar.pdf}
    \caption{Competition Counts in Full Set and Subset}
    \label{fig:counts}
\end{figure}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.5\textwidth]{AnonymousSubmission/LaTeX/images/Fullset_Counts_Bar.pdf}
    \caption{Counts of Categories within Each Competition Type in Full Set}
    \label{fig:counts}
\end{figure}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.5\textwidth]{AnonymousSubmission/LaTeX/images/Twosets_Category_Pie.pdf}
    \caption{Category Distribution}
    \label{fig:counts}
\end{figure}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.35\textwidth]{AnonymousSubmission/LaTeX/images/Twosets_ProblemType_Ring.pdf}
    \caption{Comparison of Problem Types}
    \label{fig:counts}
\end{figure}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.5\textwidth]{AnonymousSubmission/LaTeX/images/Fullset_Category_Heatmap.pdf}
    \caption{Full set Heatmap}
    \label{fig:counts}
\end{figure}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.5\textwidth]{AnonymousSubmission/LaTeX/images/Subset_Category_Heatmap.pdf}
    \caption{Subset Heatmap}
    \label{fig:counts}
\end{figure}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.5\textwidth]{AnonymousSubmission/LaTeX/images/Twosets_Num_Soultions_Bar.pdf}
    \caption{Average Number of Solutions by Competition Type}
    \label{fig:counts}
\end{figure}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.5\textwidth]{AnonymousSubmission/LaTeX/images/Fullset_Avg_Tokens_Scatter.pdf}
    \caption{Frequency of AVG Solution Tokens in Full Set}
    \label{fig:counts}
\end{figure}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.4\textwidth]{AnonymousSubmission/LaTeX/images/Subset_Avg_Tokens_Scatter.pdf}
    \caption{Frequency of AVG Solution Tokens in Subset}
    \label{fig:counts}
\end{figure}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.4\textwidth]{AnonymousSubmission/LaTeX/images/Twosets_Avg_Tokens_Scatter.pdf}
    \caption{AVG Solution Token Counts by Category}
    \label{fig:counts}
\end{figure}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.4\textwidth]{AnonymousSubmission/LaTeX/images/Twosets_Difficulty_Scatter.pdf}
    \caption{Frequency of Difficulty Levels by Category}
    \label{fig:counts}
\end{figure}

==> table/dataset.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor{lightgray}
\textbf{Dataset} & \textbf{Number of problems} & \textbf{Number of Solutions} & \textbf{Difficulty Level} & \textbf{Problem Type} \\
\hline
Our Dataset & 6469 & 14223 & Middle School to Olympic & Multiple choice, Proof, Open-end \\
\hline
GSM8K & 8792 & 8792 & High School & Open-end \\
\hline
MATH & 12500 & 12500 & Middle School & Open-end \\
\hline
\end{tabular}
\caption{Comparison of different math problem datasets}
\label{tab:my-table}
\end{table}

==> table/q2.tex <==

\begin{table}[ht]
% \centering\caption{k's impact on Correctness Acc. (\#samples varies in 400, 154, 42, 8)}
\caption{Correctness Ratio ($C$) across different models with varying numbers of provided reference solutions ($k$).}

    \begin{tabular}{lcccc}
        \hline
        \textbf{Model} & \textbf{$k=1$} & \textbf{$k=2$} & \textbf{$k=3$} & \textbf{$k=4$}  \\
        \hline
        Gemini-1.5-Pro & \textbf{68.00} & \textbf{70.78} & \textbf{78.57} & \textbf{100}  \\
        Llama-3-70B & 55.00 & 66.23 & 64.29 & 75.00\\
        Claude-3-Opus & 55.00 & 66.88 & 76.19 & 75.00 \\
        Qwen1.5-72B & 43.75 & 55.19 & 57.14 & 37.50 \\
        DeepSeek-V2 & 61.00 & 66.88 & 71.32 & 75.00 \\
        GPT-4o & 58.25 & 64.94 & 66.67 & 75.00\\
        Yi-1.5-34B & 42.75 & 42.21 & 47.62 & 50.00 \\
        Mixtral-8x22B & 53.50 & 60.39 & 64.28 & 62.50  \\
        Deepseek-Math & 35.50 & 40.91 & 52.38 & 50.00\\
        Internlm2-Math & 38.00 & 42.21 & 47.62 & 62.50\\
        \hline
    \end{tabular}
\label{tab:correctness}
\end{table}

% \begin{table}[ht]
% \centering\caption{k's impact on Novelty Acc}
%     \begin{tabular}{lcccc}
%         \hline
%         \textbf{Model} & \textbf{k = 1} & \textbf{k = 2} & \textbf{k = 3} & \textbf{k = 4}  \\
%         \hline
%         Gemini-1.5-Pro & 65.00 & 67.53 & 76.19 & 100 \\
%         Llama-3-70B & 46.50 & 54.55 & 45.24 & 62.50\\
%         Claude-3-Opus & 42.25 & 48.70 & 47.62 & 62.50 \\
%         Qwen1.5-72B & 33.75 & 33.77&26.19 & 25.00 \\
%         DeepSeek-V2 & 33.50& 25.97 & 23.81 & 37.50 \\
%         GPT-4o & 31.50 & 27.27 & 28.57 & 25.00 \\
%         Yi-1.5-34B & 29.75 & 25.97 & 35.71 & 25.00 \\
%         Mixtral-8x22B & 30.00 & 21.43 & 21.43 & 37.50  \\
%         Deepseek-Math & 12.25 & 12.34 & 16.67 & 12.50\\
%         Internlm2-Math & 12.50 & 11.69 & 7.14 & 12.50\\
%         \hline
%     \end{tabular}
% \label{tab:novelty}
% \end{table}


% \begin{table}[ht]
% \centering\caption{k's impact on Novelty/correctness ratio}
%     \begin{tabular}{lcccc}
%         \hline
%         \textbf{Model} & \textbf{k = 1} & \textbf{k = 2} & \textbf{k = 3} & \textbf{k = 4}  \\
%         \hline
%         Gemini-1.5-Pro &  95.59 & 95.41 & 96.97 & 100\\
%         Llama-3-70B & 84.55 & 82.35& 70.37 & 83.33 \\
%         Claude-3-Opus &  76.82 & 72.82 & 62.50 & 83.33\\
%         Qwen1.5-72B & 77.14&61.18&45.83&66.67 \\
%         DeepSeek-V2 & 54.92 & 38.83 & 33.33 & 50.00 \\
%         GPT-4o & 54.08 & 42.00 & 42.86 & 33.33 \\
%         Yi-1.5-34B & 69.59 & 61.54 & 75.00 & 50.00 \\
%         Mixtral-8x22B & 56.07 & 35.48 & 33.33 & 60.00  \\
%         Deepseek-Math & 34.51 & 30.16 & 31.82 & 25.00 \\
%         Internlm2-Math & 32.89 & 27.69 & 15.00 & 20.00 \\
%         \hline
%     \end{tabular}
% \label{tab:novelty_correctness_ratio}
% \end{table}

% \begin{table}[ht]
% \centering\caption{n-k's impact on Correctness Acc. (\#samples varies in 400, 154, 42, 8)}
%     \begin{tabular}{lcccc}
%         \hline
%         \textbf{Model} & \textbf{n-k=0} & \textbf{n-k=1} & \textbf{n-k=2} & \textbf{n-k=3}  \\
%         \hline
%         Gemini-1.5-Pro & 71.50 & 63.64 & 78.57 & 62.50  \\
%         Llama-3-70B & 58.00 & 61.69 & 57.14 & 50.00 \\
%         Claude-3-Opus & 61.75 & 55.19 & 57.14 & 75.00 \\
%         Qwen1.5-72B & 49.00 & 43.51 & 47.62 & 37.50 \\
%         DeepSeek-V2 & 63.75 & 62.34 & 59.52 & 87.50 \\
%         GPT-4o & 61.25 & 58.44 & 61.90 & 75.00\\
%         Yi-1.5-34B & 43.00 & 39.61 & 52.38 & 50.00 \\
%         Mixtral-8x22B & 56.00 & 56.49 & 50.00 & 75.00  \\
%         Deepseek-Math & 37.75 & 37.66 & 42.86 & 62.50 \\
%         Internlm2-Math & 40.00 & 39.61 & 35.71 & 75.00 \\
%         \hline
%     \end{tabular}
% \label{tab:correctness2}
% \end{table}

% \begin{table}[ht]
% \centering\caption{n-k's impact on Novelty Acc}
%     \begin{tabular}{lcccc}
%         \hline
%         \textbf{Model} & \textbf{n-k=0} & \textbf{n-k=1} & \textbf{n-k=2} & \textbf{n-k=3}  \\
%         \hline
%         Gemini-1.5-Pro & 68.00 & 61.04 & 78.57 & 62.50 \\
%         Llama-3-70B & 47.00 & 52.60 & 50.00 & 50.00 \\
%         Claude-3-Opus & 45.50 & 40.26 & 52.38 & 50.00 \\
%         Qwen1.5-72B & 33.50 & 30.52 & 40.48 & 25.00 \\
%         DeepSeek-V2 & 30.50& 33.77 & 21.43 & 50.00 \\
%         GPT-4o & 29.00 & 31.17 & 35.71 & 37.50 \\
%         Yi-1.5-34B & 29.75 & 25.97 & 30.95 & 37.50 \\
%         Mixtral-8x22B & 26.00 & 29.87 & 26.19 & 50.00  \\
%         Deepseek-Math & 13.25 & 9.74 & 11.90 & 37.50\\
%         Internlm2-Math & 11.50 & 14.29 & 7.14 & 12.50\\
%         \hline
%     \end{tabular}
% \label{tab:novelty2}
% \end{table}


% \begin{table}[ht]
% \centering\caption{n-k's impact on Novelty/correctness ratio}
%     \begin{tabular}{lcccc}
%         \hline
%         \textbf{Model} & \textbf{n-k=0} & \textbf{n-k=1} & \textbf{n-k=2} & \textbf{n-k=3}  \\
%         \hline
%         Gemini-1.5-Pro &  95.10 & 95.92 & 100 & 100\\
%         Llama-3-70B & 81.03 & 85.26 & 87.50 & 100 \\
%         Claude-3-Opus & 73.68 & 72.94 & 91.67 & 66.67 \\
%         Qwen1.5-72B & 68.37 & 70.15 & 85.00 & 66.67 \\
%         DeepSeek-V2 & 47.84 & 54.17 & 36.00 & 57.14 \\
%         GPT-4o & 47.35 & 53.33 & 57.69 & 50.00 \\
%         Yi-1.5-34B & 46.43 & 52.87 & 52.38 & 66.67 \\
%         Mixtral-8x22B & 56.07 & 35.48 & 33.33 & 60.00  \\
%         Deepseek-Math & 35.10 & 25.86 & 27.78 & 60.00 \\
%         Internlm2-Math & 32.89 & 27.69 & 15.00 & 20.00 \\
%         \hline
%     \end{tabular}
% \label{tab:novelty_correctness_ratio2}
% \end{table}

\begin{table}[ht]
\caption{Novelty/Correctness Ratio ($N/C$) for different models based on the degree of solution availability ($n-k$). Higher values of $n-k$ indicate scenarios with fewer provided solutions, which are easier for the LLM.}
    \begin{tabular}{lccc}
        \hline
        \textbf{Model} & \textbf{$n-k=2$} & \textbf{$n-k=1$} & \textbf{$n-k=0$} \\
        \hline
        Gemini-1.5-Pro & \textbf{100} & \textbf{95.92} & \textbf{95.10} \\
        Llama-3-70B & 87.50 & 85.26 & 81.03 \\
        Claude-3-Opus & 91.67 & 72.94 & 73.68 \\
        Qwen1.5-72B & 85.00 & 70.15 & 68.37 \\
        DeepSeek-V2 & 36.00 & 54.17 & 47.84 \\
        GPT-4o & 57.69 & 53.33 & 47.35 \\
        Yi-1.5-34B & 52.38 & 52.87 & 46.43 \\
        Mixtral-8x22B & 33.33 & 35.48 & 56.07 \\
        Deepseek-Math & 27.78 & 25.86 & 35.10 \\
        Internlm2-Math & 15.00 & 27.69 & 32.89 \\
        \hline
    \end{tabular}
\label{tab:novelty_correctness_ratio2}
\end{table}




